Ride Sharing with a Vehicle of Unlimited Capacity

A ride sharing problem is considered where we are given a graph, whose edges are equipped with a travel cost, plus a set of objects, each associated with a transportation request given by a pair of origin and destination nodes. A vehicle travels through the graph, carrying each object from its origin to its destination without any bound on the number of objects that can be simultaneously transported. The vehicle starts and terminates its ride at given nodes, and the goal is to compute a minimum-cost ride satisfying all requests. This ride sharing problem is shown to be tractable on paths by designing a $O(h \log h+n)$ algorithm, with $h$ being the number of distinct requests and with $n$ being the number of nodes in the path. The algorithm is then used as a subroutine to efficiently solve instances defined over cycles, hence covering all graphs with maximum degree $2$. This traces the frontier of tractability, since $\bf NP$-hard instances are exhibited over trees whose maximum degree is $3$.

==> conclusion.tex <==
We have consider a ride sharing problem with a vehicle of unlimited capacity, by completely classifying its complexity w.r.t.~the underlying
network topology. The main result is a $O(|C| \log |C|)$ algorithm for computing an optimal ride over paths, with $C$ denoting the set of the
available requests.
%
Our results have a wide spectrum of applicability, in particular, to find optimal rides whenever it is a-priori known that the number of
objects to be transported does not exceed the capacity of the vehicle.

In fact, computing an optimal ride might be not enough in some applications. Indeed, especially in the context of transportation of passengers
(such as in \emph{dial-a-ride} problems~\cite{DRP}), the human perspective tend to introduce further requirements leading to balance user
inconvenience against minimizing routing costs; in particular, the time comparison of the chosen route with respect to the shortest path to a
destination is a widely-used measure of customer satisfaction in (the related) \emph{school bus routing problems}~\cite{Park2010311}.
Accordingly, an interesting avenue for further research is to adapt our solution algorithms by taking into account fairness requirements.
%
Finally, we stress here that another interesting technical question is to assess whether, in our basic optimization setting, further
tractability results can be established by focusing on requests of special kinds, for instance, on requests where the starting and terminating
nodes precisely identify the endpoints of some edge. In this latter case, it would be interesting to analyze the complexity over trees (which
emerged to be intractable with arbitrary requests) and, more generally, over graphs having bounded treewidth.

